On Abel-Jacobi Maps of Lagrangian Families

We study in this article the cohomological properties of Lagrangian families on projective hyper-K\"ahler manifolds. First, we give a criterion for the vanishing of Abel-Jacobi maps of Lagrangian families. Using this criterion, we show that under a natural condition, if the variation of Hodge structures on the degree $1$ cohomomology of the fibers of the Lagrangian family is maximal, its Abel-Jacobi map is trivial. We also construct Lagrangian families on generalized Kummer varieties whose Abel-Jacobi map is not trivial, showing that our criterion is optimal.

==> AnExample.tex <==
%Need to show the two lemmas and show that the deformation is full. 
In this section, we shall give a full lagrangian family in a generalized Kummer variety~\cite{Beauville} of dimension $4$ whose base is not rationally connected. 

Let $E$ be an elliptic curve endowed with a complex multiplication by $\omega:=e^{2\iota\pi/3}$. Consider on $A:=E\times E$, the automorphism $\eta: A\to A$ defined by $(x_1,x_2)\mapsto (x_1,\omega x_2)$. Let $X:=K_2(A)\subset Hilb^3(A)$ be the generalised Kummer variety of dimension $4$.

Let $a\in A$, we construct a subvariety $L_a\subset X$ by the following procedures. First consider the image $I_a$ of the set $\{(x+a, \eta(x)-a, \eta^2(x)): x\in A\}\subset A\times A\times A$ under the symmetric map $A^3\to Sym^3(A)$. Since $Hilb^3(A)$ is a desingularisation of $Sym^3(A)$~\cite{Fogarty}, we let $L_a$ be the strict transformation of $I_a$ of this desingularisation. $L_a$ lies in $X\subset Hilb^3(A)$ by construction. We will denote general elements in $X=K_2(A)$ as $(z_1)+(z_2)+(z_3)$ with $z_1+z_2+z_3=0$ in $A$. Therefore, $L_a$ is the closure of 
\[\{(x+a)+(\eta(x)-a)+(\eta^2(x)): x\in A\}\subset X.
\]

\begin{lmm}\label{GeneralFibersAreAbelian}
Let $a=(a_1,a_2)\in E\times E=A$. If $6a_1\neq 0$, then $L_a$ is smooth and is an abelian variety.
\end{lmm}
\begin{prf}
If $6a_1\neq 0$, then for any $x\in A$, the three points $x+a$, $\eta(x)-a$ and $\eta^2(x)$ are distinct. Therefore, $I_a$ does not meet the image of \begin{equation}\label{DefinitionOfDelta}
    \Delta:=\{(z_1, z_2, z_3)\in A^3: \exists i\neq j, z_i=z_j\}
\end{equation} 
in $Sym^3(A)$. Since $Hilb^3(A)$ and $Sym^3(A)$ are isomorphic outside the image of $\Delta$ (see~\cite{Fogarty}), we conclude that $L_a\cong I_a$. Furthermore, for such $a$, the map 
\[\begin{array}{ccc}
   A &\to  & I_a\cong L_a \\
    x & \mapsto & (x+a)+(\eta(x)-a)+(\eta^2(x))
\end{array}
\]
is a bijection. Indeed, if $x, x'\in A$ map to the same point in $I_a$, i.e., $(x+a)+(\eta(x)-a)+(\eta^2(x))=(x'+a)+(\eta(x')-a)+(\eta^2(x'))$, then $x$ and $x'$ should satisfy one of the six systems of equations. Therefore, $L_a\cong I_a\cong A$ is smooth and is an abelian variety.
\end{prf}

\begin{lmm}\label{ThisIsALagrangianFamily}
For any $a\in A$, $L_a\subset X$ is a lagrangian subvariety.
\end{lmm}
\begin{prf}
Recall from~\cite{Beauville} the definition of the holomorphic $2$-form $\sigma_X$ on $X$. Let $\Delta$ be defined as in (\ref{DefinitionOfDelta}). and $\delta:=\{(z,z,z)\in A^3: z\in A\}$. Let $A^3_*$ (resp. $\Delta_*$) be defined by $A^3$ (resp. $\Delta$) deprived $\delta$. Let $Hilb^3(A)_*$ be $Hilb^3(A)$ deprived the preimage of $\delta$. Then we have the following commutative diagram~\cite{Beauville}:
\begin{equation}
    \begin{tikzcd}
    & & Bl_{\Delta_*}(A^3_*) \arrow{r}{\phi} \arrow{d}{p} & A^3\arrow{d}{\pi} \\
    X=K_2(A)\arrow[hookrightarrow]{r} & Hilb^3(A)\arrow[hookleftarrow]{r} & Hilb^3(A)_*\arrow{r}{\psi} & Sym^3(A)
    \end{tikzcd}.
\end{equation}
The the $2$-form $\sigma_X$ is the restriction of a $2$-form $\sigma$ on $Hilb^3(A)$ such that
\begin{equation}\label{DefinitionOfSigmaX}
    p^*\sigma=\phi^*(pr_1^*\sigma_A+pr_2^*\sigma_A+pr_3^*\sigma_A),
\end{equation}
where $pr_i: A^3\to A$ is the projection and $\sigma_A$ is a nonzero holomorphic $2$-form on $A$ (unique up to coefficients). In order to show that $L_a$ is lagrangian, in view of (\ref{DefinitionOfSigmaX}), it is equivalent to showing that 
\begin{equation}\label{LagrangianEquation}
    f_1^*\sigma_A+f_2^*\sigma_A+f_3^*\sigma_A=0,
\end{equation}
where $f_1: x\mapsto x+a$, $f_2: x\mapsto \eta(x)-a$ and $f_3: x\mapsto \eta^2(x)$. But the left-hand-side of (\ref{LagrangianEquation})
is $\sigma_A+\omega\sigma_A+\omega^2\sigma_A$, which is zero, as desired.
\end{prf}

\begin{lmm}
Let $a, a'\in A$. Assume that one of $a, a'$ lies in the open dense subset $(E\setminus\{0\})\times E\subset A$, $L_a=L_{a'}$. If $a\neq a'$, then $L_a\neq L_{a'}$.
\end{lmm}
\begin{prf}
Let $a=(a_1,a_2)$ and $a'=(a_1',a_2')$. May assume $a_1\neq 0$. Assume $L_a=L_{a'}$ and we show that $a=a'$. By assumption, for (almost) all $x\in A$, one may find $x'\in A$ such that
$(x+a)+(\eta(x)-a)+(\eta^2(x))=(x'+a')+(\eta(x')-a')+(\eta^2(x'))$, which means that one of the six systems of equations of the form
\[\left\{\begin{array}{ccc}
        x+a & = & x'+a'  \\
        \eta(x)-a  &= & \eta(x')-a' \\
        \eta^2(x) &= &\eta^2(x')
    \end{array}\right.\]
holds. Check them one-by-one, we find that, unless $a=a'$, each of the six systems has solutions only for finitely many (maybe none) $x\in A$, subject to the condition that $a_1\neq 0$. Therefore, we are forced to have $a=a'$.
\end{prf}

Therefore, we constructed a lagrangian family (Lemma~\ref{ThisIsALagrangianFamily}) parametrized by (a variety birational to) $A$. This family is a full family. Indeed, by Lemma~\ref{GeneralFibersAreAbelian}, the general fibers are smooth and are abelian varieties of dimension $2$. Deformation Theory of \emph{smooth} lagrangian subvarieties (see~\cite{VoisinLag}) shows that universal space of these smooth lagrangian subvarieties is of dimension $h^0(L_b,\Omega_{L_b})=2$. But the base space $A$ has already dimension $2$. The base space is not rationally connected since it is (birational to) the abelian surface $A$.
